When, why, and how do diffusion posterior samplers fail? A finite-sample lens

Diffusion models have excellent capacity to model complex distributions of natural data, which has made them a popular and effective choice for posterior sampling in imaging inverse problems. Existing methods can incorporate any measurement model at inference time but must use an inexact approximation for the likelihood at intermediate timesteps for computational tractability. Although these approximations can often work well empirically, their downstream effect on the sampled posterior is poorly understood and can result in unexplained failures. To understand when, why, and how these likelihood approximations propagate to erroneous posterior distributions, we introduce a finite-sample perspective on posterior sampling that approximates the posterior to arbitrary precision as training set size tends towards infinity, for any forward model and prior distribution. Using this finite-sample lens, we observe that popular posterior sampling approximations tend to under- or over-estimate the spread of the posterior at intermediate timesteps, causing downstream consequences including sensitivity to early stopping time, inaccurate relative weighting of posterior modes, and hallucination, both of prior modes that are not in the posterior and likelihood modes that are not supported by the prior. Moreover, we find that the cause of these posterior errors requires neither a nonlinear measurement model nor a multimodal posterior, but can arise solely due to a multimodal prior and inaccurate posterior spread at intermediate sampling times. Our finite-sample posterior sampling approach is agnostic to the type of likelihood approximation and the type of (linear or nonlinear) forward model, and can thus serve as a drop-in diagnostic to evaluate the accuracy and failure modes of existing and future posterior samplers.

==> style.tex <==
% The abstract paragraph should be indented \nicefrac{1}{2}~inch (3~picas) on both the left- and right-hand margins. Use 10~point type, with a vertical spacing (leading) of 11~points. The word \textbf{Abstract} must be centered, bold, and in point size 12. Two line spaces precede the abstract. The abstract must be limited to one paragraph.

% 9 pages long, not including ack, refs, and appendix

% All headings should be lower case (except for first word and proper nouns), flush left, and bold.

% The \verb+natbib+ package will be loaded for you by default.  Citations may be author/year or numeric, as long as you maintain internal consistency.  As to the format of the references themselves, any style is acceptable as long as it is used consistently.

% If you wish to load the \verb+natbib+ package with options, you may add the
% following before loading the \verb+neurips_2026+ package:
% \begin{verbatim}
%    \PassOptionsToPackage{options}{natbib}
% \end{verbatim}


% If \verb+natbib+ clashes with another package you load, you can add the optional
% argument \verb+nonatbib+ when loading the style file:
% \begin{verbatim}
%    \usepackage[nonatbib]{neurips_2026}
% \end{verbatim}


% All tables must be centered, neat, clean, and legible.  The table number and title always appear before the table.  See Table~\ref{sample-table}.

% Place one line space before the table title, one line space after the table title, and one line space after the table. The table title must be lower case (except for the first word and proper nouns); tables are numbered consecutively. No vertical rules

% \begin{table}
%   \caption{Sample table caption. Explain what the table shows and add a key take-away message to the caption.}
%   \label{sample-table}
%   \centering
%   \begin{tabular}{lll}
%     \toprule
%     \multicolumn{2}{c}{Part}                   \\
%     \cmidrule(r){1-2}
%     Name     & Description     & Size ($\mu$m) \\
%     \midrule
%     Dendrite & Input terminal  & $\approx$100     \\
%     Axon     & Output terminal & $\approx$10      \\
%     Soma     & Cell body       & up to $10^6$  \\
%     \bottomrule
%   \end{tabular}
% \end{table}

% Please prepare submission files with paper size ``US Letter,'' and not, for example, ``A4.''


% You can check which fonts a PDF files uses.  In Acrobat Reader, select the menu Files$>$Document Properties$>$Fonts and select Show All Fonts. You can also use the program \verb+pdffonts+ which comes with \verb+xpdf+ and is available out-of-the-box on most Linux machines.

% If your file contains type 3 fonts or non embedded TrueType fonts, we will ask you to fix it.

% A number of width problems arise when \LaTeX{} cannot properly hyphenate a line. Please give LaTeX hyphenation hints using the \verb+\-+ command when necessary.

% References follow the acknowledgments in the camera-ready paper. Use unnumbered first-level heading for the references. Any choice of citation style is acceptable as long as you are consistent. It is permissible to reduce the font size to \verb+small+ (9 point) when listing the references. Note that the Reference section does not count towards the page limit.

==> tikz-plots/fsr_tv/fsr_tv.tex <==
% Standalone preview wrapper.
\input{../tikz_preamble}
\pgfplotsset{compat=1.18}
\usepackage{natbib}
\usetikzlibrary{calc}
\begin{document}
\pagestyle{empty}
\input{fsr_tv_body}
\end{document}


==> tikz-plots/image_grid/image_grid.tex <==
% Standalone preview wrapper. The figure itself lives in image_grid_body.tex
\input{../tikz_preamble}
\pgfplotsset{compat=1.18}
\usepackage{graphicx}
\usepackage{natbib}
\usetikzlibrary{calc}
\begin{document}
\pagestyle{empty}
\input{image_grid_body}
\end{document}


==> tikz-plots/image_grid_error/image_grid_error.tex <==
% Standalone preview wrapper. Figure body lives in image_grid_error_body.tex
\input{../tikz_preamble}
\pgfplotsset{compat=1.18}
\usepackage{natbib}
\usetikzlibrary{calc}
\begin{document}
\pagestyle{empty}
\input{image_grid_error_body}
\end{document}


==> tikz-plots/quadratic_grid/quadratic_grid.tex <==
% Standalone preview wrapper. The figure itself lives in quadratic_grid_body.tex
\input{../tikz_preamble}
\pgfplotsset{compat=1.18}
\usepackage{graphicx}
\usepackage{natbib}
\usetikzlibrary{calc}
\begin{document}
\pagestyle{empty}
\input{quadratic_grid_body}
\end{document}

